Draco 2: An Extensible Platform to Model Visualization Design

Draco introduced a constraint-based framework to model visualization design in an extensible and testable form. It provides a way to abstract design guidelines from theoretical and empirical studies and applies the knowledge in automated design tools. However, Draco is challenging to use because there is limited tooling and documentation. In response, we present Draco 2, the successor with (1) a more flexible visualization specification format, (2) a comprehensive test suite and documentation, and (3) flexible and convenient APIs. We designed Draco 2 to be more extensible and easier to integrate into visualization systems. We demonstrate these advantages and believe that they make Draco 2 a platform for future research.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> draft.tex <==
%%%%% abstract %%%%%%%%

Visualization recommendation engines have the potential to enhance data exploration by intelligently suggesting suitable visualizations for users' data and tasks. However, integrating these recommendation engines into applications or systems is challenging, as most of the existing solutions are monolithic and opaque, lacking sufficient modularity, documentation, and explainability, hindering seamless integration.  Draco introduces an extensible, constraint-based framework for representing visualization design knowledge, but is still challenging to use in practice due to the limited tooling and documentation it comes with.
We present Draco 2, a successor with a modular architecture and updated developer experience. It runs in Python and browsers, enabling easy integration into applications. Building on Draco's knowledge base, using an extensible chart specification format, Draco 2 supports multi-view and multi-layer designs. The testing and tuning infrastructure we provide facilitates examining and tailoring Draco 2's knowledge base, converting our recommendation engine into a comprehensive platform that is able to process visualization constraints, yield conformant specifications, and render the specified graphics. We show three cases that demonstrate Draco 2 reasoning about and recommending visualizations.


%%%%%%% Intro %%%%%%%%

The field of visualization recommendation is complex and ever-changing~\cite{Zhu2020survey}. Technological advancements and research progress in other disciplines where data visualization is an essential tool keep inspiring novel recommendation techniques, the emergence of new data types and increasingly large datasets motivate the enhancement of visualization design knowledge while the constant shift in user needs and preferences call for fresh visualization recommendation experiences.

Early visualization recommendation research used rule-based approaches, later studies applied machine learning and hybrid techniques, while recent efforts have focused on crafting interactive systems that provide personalized recommendations based on user feedback. While approaches have varied and will continue to vary over time, visualization recommendation research consistently builds upon current, established visualization design knowledge and best practices.

Moritz et al.~\cite{Moritz2018FormalizingVD} proposed Draco as a formal model to capture this ever-growing visualization design knowledge as logical facts and developed a framework to shift abstract, theoretical visualization design guidelines to concrete, extensible formulations.

Even though its knowledge representation framework can keep up with the expanding design rules over time, Draco falls short in certain aspects. A notable limitation of Draco is that the visualization specifications it suggests are strictly tied to  Vega-Lite, restricting the potential design space of recommendations to single-view visualizations. Furthermore, as a result of the limited documentation, test coverage and tooling Draco comes with, it is difficult to be adopted as a library. The inability to be integrated into emerging projects hinders Draco to be a truly instrumental tool for future research.

We hope to do more than remedy the aforementioned shortcomings with the introduction of Draco 2; we aspire to construct a durable platform for sustained progress in future research through key foundations of the project.

Thorough, actively-maintained documentation is essential for a future-proof platform, to ensure that the supported features are easily accessible for builders. Draco 2 offers comprehensive documentation covering its core modules and its lower-level building blocks alike comprising hands-on examples to provide practical guidance for users. 

Incorporating a new tool into one's system can be deterred by uncertainties regarding the tool's stability. With 100\% unit test coverage of our codebase, we aim to ensure the reliability of the platform and make Draco 2 suitable for adoption. 

An even more frequent reason why a tool stays unembraced is incompatibility with the target project's stack. Draco 2 is written in Python, but it comes with a server component exposing its capabilities through a REST API, making it seamless to interface with it. Furthermore, we provide a WebAssembly distribution of the entire recommendation engine, meaning that Draco 2 can run natively in any modern browser.

When maintaining a knowledge base about visualization design guidelines and having recommendations generated based on these, it is essential to be able to interpret how the declared rules affect the outputs. Draco 2 provides a debugging platform for this.



%%%%%%%% related work %%%%%%%%%%%

Draco~\cite{Moritz2018formalizing} is a framework for automated visualization design. 
At its core, Draco models visualizations as a set of logical facts and represents visualization design knowledge as hard and soft constraints. 

Automated visualization tools use specification languages to describe and synthesize visualization designs. Mackinlay’s APT~\cite{Mackinlay1986automating} system automatically ranks encoding choices based on the \textit{expressiveness} and \textit{effectiveness} criteria. Tableau's ShowMe~\cite{Mackinlay2007showme} suggests specific encodings with heuristic rules. Voyager’s~\cite{Wongsuphasawat2015voyager,Wongsuphasawat2017voyager2} CompassQL~\cite{Wongsuphasawat2016towards} and Draco both build on the Vega-Lite~\cite{Satyanarayan2017vegalite} grammar and combine rules that model fine-grained design knowledge with hand-tuned scores. In Draco 2, we re-design the logical representation to a generalized and extended chart specification format that is extensible and renderer-agnostic. With such a format, we support multiple views and view composition.

\section{Demonstration of Draco~2 as a modeling tool}
% Peter
% TODO: make sure we are objective in everyting we say
% TODO: add more details about why and what we do
% TODO: what do we learn from the things we did
We demonstrate Draco~2's capabilities as an effective tool to generate recommendations, explore and adapt the knowledge base. 
We created a Jupyter Notebook\footnote{\href{https://dig.cmu.edu/draco2/applications/design_space_exploration.html}{dig.cmu.edu/draco2/applications/design\_space\_exploration.html}} that explores the visualization design space of the Seattle weather dataset\footnote{\href{https://cdn.jsdelivr.net/npm/vega-datasets@v1.29.0/data/seattle-weather.csv}{cdn.jsdelivr.net/npm/vega-datasets@v1.29.0/data/seattle-weather.csv}}, and a guide for debugging recommendation results\footnote{\href{https://dig.cmu.edu/draco2/applications/debug_draco.html}{dig.cmu.edu/draco2/applications/debug\_draco.html}}.

\subsection{Exploring Existing Knowledge Base}
\textbf{Iterating the partial specification query:} 
We start with only the raw dataset input, modeling the common first step in visual data exploration. We load the dataset and generate its schema (name of the columns, their data types and key statistical properties) as logical facts with the \mintinline{python}{schema_from_dataframe} function. Then, for the recommendation query, we concatenate the schema with \mintinline{prolog}{entity(view,root,v0)} and \mintinline{prolog}{entity(mark,v0,m0).}, aiming to generate single-view, single-mark visualizations. We generate and render the top recommendations using the \mintinline{python}{complete_spec} and the \mintinline{python}{AltairRenderer}. 
The top five results encode the count of records because in general using less encoding is preferred, and they represent an overview given that less information is specified by the query. Two of them encode a non-aggregated second field, \mintinline{latex}{weather}, via columnar faceting. 

After an initial overview and inspiration, we explore how Draco~2 can be used to creating more targeted outputs. To constrain the desired design space, we extend the base input specification with additional facts to include \mintinline{latex}{date} temporal field and \mintinline{latex}{temp_max} numeric field in the target results. We also specifies a preference for column-faceted charts, while allowing our tool to determine other details. As a result, we obtain charts faceted by the \mintinline{latex}{weather} field since it is a categorical variable with low cardinality. And the faceted scatter plot without binning is preferred to the faceted tick chart where the \mintinline{latex}{temp_max} field is binned. Draco~2 successfully produces visualizations from partial specification based on the fundamental visualization design guidelines expressed by our knowledge base. We can test more input variations and compare their costs, for example, by forbidding the facet and adding another encoding the \mintinline{latex}{weather} field can be encoded as a color channel. 

% We set off by investigating what visualizations our tool recommends having only the raw dataset as a starting point, thereby modeling a common first step of visual data exploration. We formed initial recommendations using a minimal input specification that contained the dataset's schema (name of the columns, their data types and key statistical properties) generated by the \mintinline{python}{schema_from_dataframe} function and two hand-written logical facts, \mintinline{prolog}{entity(view,root,v0)} and \mintinline{prolog}{entity(mark,v0,m0).} aiming to generate single-view, single-mark visualizations. We use the \mintinline{python}{complete_spec} method to enumerate the top five visualizations (ranked by model costs computed by Clingo), then we transform them from Draco~2 specifications to Vega-Lite format via the \mintinline{python}{AltairRenderer}. Subsequently, we display the Vega-Lite specifications using the Jupyter environment's \mintinline{python}{display} method. Although the generated recommendations are valid, all five of them encode the count of records and only two of them give insight into a non-aggregated field, \mintinline{latex}{weather} via columnar faceting. Furthermore, two recommendation pairs are rendered into identical Vega-Lite specifications, although their underlying Draco~2 specifications are different. Considering the first and the second chart, their Draco~2 specification differs by a single logical fact: the former has \mintinline{prolog}{attribute(task,root,summary)} while the latter has \mintinline{prolog}{attribute(task,root,value)}. Since the Vega-Lite-based renderer ignores this custom attribute, the semantically different Draco~2 specifications yield identical visuals.

% Observing the redundancy of the information encoded by the produced specifications, we explore how Draco~2 can be used for creating more targeted outputs. To better define the desired design space for recommendations, we extend the base input specification with additional facts, ensuring the inclusion of the \mintinline{latex}{date} temporal field and \mintinline{latex}{temp_max} numeric field in the resulting recommendations. 
% We also specified a preference for column-faceted charts, while allowing our tool to determine other details to investigate the dataset field Draco~2 identifies as appropriate for faceting. We obtain column-faceted charts along the \mintinline{latex}{weather} field, learning that a categorical variable is deemed as the most suitable to encode. The recommendations feature charts using point mark for specifications without binning and tick mark for outputs where the \mintinline{latex}{temp_max} field is binned. These demonstrate Draco~2's capability to produce valid visualizations from partial specification, adherent to the fundamental visualization design guidelines our knowledge base encompasses.

\textbf{Inspecting the Knowledge Base:}
To perform a more thorough analysis of the recommendations and to validate them against the design preferences (soft constraints) defined in the knowledge base, we employ Draco~2's debugger module. The \mintinline{python}{DracoDebug} module generates a Pandas \mintinline{latex}{DataFrame} containing the recommendations, the violated soft constraints, and their associated weights. We use \mintinline{python}{DracoDebugPlotter} to investigate the violation vector and weights interactively. We observe that only a small subset of the defined soft constraints (19 out of 147) impact the recommended charts due to the overlap between them.
%, caused by the fact that we defined that we wish to see only such recommendations which encode the \mintinline{latex}{date} and \mintinline{latex}{temp_max} fields.

Finally, we exhibit how we can explore a wider space of possible visualizations by adapting the knowledge base and we investigate the soft constraints impacting the produced recommendations by utilizing the debugger module once again. We specify a list of marks \mintinline{python}{["point", "bar", "line", "rect"]}, fields \mintinline{python}{["weather", "temp_min", "date"]} and encoding channels \mintinline{python}{["color", "shape", "size"]} and we extend the knowledge base temporarily with programmatically generated facts from the three-way cross product of them with the goal of obtaining a variety of charts. We learn that Draco~2 employs binning, faceting, stacking, and aggregations such as count and mean in an attempt to recommend meaningful visualizations. We also observe that some mark-field-channel combinations such as \mintinline{python}{("line", "date", "size")} do not yield any recommendations due to violating a hard-constraint, \mintinline{prolog}{size_without_point_text} in this case, defining that encoding data using the size channel only works when using point or text as the mark. Analyzing the entire output with the debugger we learn that 37 of the defined 147 soft constraints influenced the recommendations, indicating that we explored a wider space of possible designs.

In conclusion, we demonstrated how Draco~2 can be used as a modeling tool by employing its modular Python API to interact with the knowledge base and perform visualization recommendation by producing completions for partial specifications. We exhibited how the completed specifications can be converted to the novel visualization specification format we introduced and we illustrated how these can be translated to Vega-Lite using the renderer we contributed. Furthermore, we presented how the debugger module aids the validation of charts as well as how it can be applied to gain insight into the soft constraints and their weights.

